Regularized Discrete Optimal Transport

This article introduces a generalization of the discrete optimal transport, with applications to color image manipulations. This new formulation includes a relaxation of the mass conservation constraint and a regularization term. These two features are crucial for image processing tasks, which necessitate to take into account families of multimodal histograms, with large mass variation across modes. The corresponding relaxed and regularized transportation problem is the solution of a convex optimization problem. Depending on the regularization used, this minimization can be solved using standard linear programming methods or first order proximal splitting schemes. The resulting transportation plan can be used as a color transfer map, which is robust to mass variation across images color palettes. Furthermore, the regularization of the transport plan helps to remove colorization artifacts due to noise amplification. We also extend this framework to the computation of barycenters of distributions. The barycenter is the solution of an optimization problem, which is separately convex with respect to the barycenter and the transportation plans, but not jointly convex. A block coordinate descent scheme converges to a stationary point of the energy. We show that the resulting algorithm can be used for color normalization across several images. The relaxed and regularized barycenter defines a common color palette for those images. Applying color transfer toward this average palette performs a color normalization of the input images.

==> sections/sec-prox-algo.tex <==
\section{Algorithms}

\paragraph{$\ell-1$ norm} Conic optimization problem (Mosek)

\paragraph{$\ell-2$ norm} Proximal-splitting with Chambolle and Pock (nunca implementado??)



Problem~\eqref{eq-relaxed-regularized-cvx} is a convex minimization. In the case $p=2$, it corresponds to a quadratic minimization, whereas in the case $p=1$ it can be cast as a conic optimization problem. They can be solved for medium-scale problem using standard interior point methods. An alternative solution is to use first order proximal scheme (see for instance~\cite{Chambolle11}), that are well tailored for such highly structured problems. 

\paragraph{Proximal Splitting.}Problem~\eqref{eq-relaxed-regularized-cvx} can be reformulated as
\eql{\label{eq-relaxed-regularized-cvx-permutation-relaxed}
	\umin{\Si} \dotp{C}{\Si} + \la \regul{G (X - \Si Y)} + \iota_{\Dd_1}(\Si) + \iota_{\Cc_\kappa}(\Si^*)
}
where $\iota_C$ is the indicator function of a convex set $C$ and we introduced the constraint sets
\begin{align*}
	\Cc_\kappa = \enscond{\Si}{\Si \geq 0, \: \Si \U \leq \kappa \U, \Si \in \RR^{N \times N}}.
\end{align*}
and $\iota_{\Dd_1}$ is the indicator function of the convex set $\Dd_1$ defined as:
\begin{align*}
	\Dd_1 = \enscond{\Si}{\Si \geq 0, \: \Si \U = \U, \Si \in \RR^{N \times N} },
\end{align*}
where every line of $\Si\in\Dd_1$ belongs to the $N$-dimensional simplex.
Problem~\eqref{eq-relaxed-regularized-cvx-permutation-relaxed} can be re-casted as a minimization of the form
\eq{ 
	\umin{\Si \in \RR^{N \times N}} F(K(\Si)) + H(\Si) 
}
\eq{
	\qwhereq
	\choice{
	K(\Si) = (\Si, G \Si Y), \quad K^*(\Si,U) = \Si + G^* U Y^*, \\
	F(\Si,U) = \la \regul{U-G X} + \iota_{\Dd_1}(\Si), \\
	H(\Si) = \dotp{C}{\Si} + \iota_{\Cc_\kappa}(\Si^*).
	}
}
%\todo{I think there are errors in $\Prox_{\ga F}$: $\la GX$ should probably be $\ga GX$ and $\la$ is lacking in $ \Prox_{\la \ga \regul{\cdot}}$. Check this. }
\paragraph{Orthogonal projection on constraint sets.}The proximal operators read
\begin{align*}
	\Prox_{\ga F}(\Si,U) &= ( \Proj_{\Dd_1}(\Si) ,\la GX + \Prox_{\ga \regul{\cdot}}(U-\la GX)) \\
	\Prox_{\ga H}(\Si) &= \left(\Proj_{\Cc_\kappa}((\Si - \ga C)^*)\right)^*
\end{align*}
where the orthogonal projection on $\Cc_\kappa$ is computed for each line $\Sigma_\ell$ of a matrix $\Si$ as
\if 0
\eq{ \Proj_{\Cc_\kappa}(\Si_l)=\left\{\begin{array}{ll} \max(0, \Si_l)&\textrm{ if }\max(0, \Si_l)\U\leq \kappa\\
\Proj_{\Dd_\kappa}(\Si_l)&\textrm{ otherwise},
\end{array}\right,
}
\fi

\eq{
 \tilde \Sigma = \Proj_{\Cc_\kappa}(\Sigma) \qwhereq \tilde\Sigma_\ell = \left\{\begin{array}{ll} \max(0, \Si_l)&\textrm{ if }\max(0, \Si_l)\U\leq \kappa\\
\Proj_{\Dd_\kappa}(\Si_l)&\textrm{ otherwise},
\end{array}\right\}
}


where $\Proj_{\Dd_\kappa}(V)$ is the projection of the line vector $V$ on the convex set $\Dd_\kappa$
\begin{align*}
	\Dd_\kappa = \enscond{V}{V \geq 0, \: V \U = \kappa }.
\end{align*}
This last projection, as well as the projection on $\Dd_1$, can be efficiently computed as detailed for instance in~\cite{duchi-projection}.

%\todo{I have removed the citation to Chen11, in fact this is a very classical problem and solutions have been published several times before (including by Bertsekas in the 80s). }

\paragraph{Proximal Operators.}Let us now recall that the proximal operator of a function $F$ is defined as 
\eq{ 
	\Prox_{\ga F}(\Si) = \uargmin{\tilde\Si} \frac{1}{2}\norm{\Si-\tilde \Si}^2 + \ga F(\tilde \Si) .
}
One can check that for $p=1$ and $p=2$, the proximal operator of $J_p$  evaluated at $U\in\RR^{N \times d}$ can be computed in closed form as:
\begin{align*}
\Prox_{\la \ga J_1({\cdot})}(U)_i&=\max\left(0,1- \frac{\la \ga}{\norm{U_i}}\right)U_i \qandq
\Prox_{\la \ga   J_2({\cdot})}(U)_i&=\frac{U_i}{1+2\ga\la}
\end{align*}
Note that being able to compute the proximal mapping of $F$ is equivalent to being able to compute the proximal mapping of $F^*$, thanks to Moreau's identity
\eq{
	\Si = \Prox_{\ga F^*}(\Si) + \ga \Prox_{F/\ga}(\Si/\ga).
}
\paragraph{Primal-dual splitting scheme.}The primal-dual algorithm of~\cite{Chambolle11} applied to our problem finally reads
\begin{align*}
	\Ga^{k+1} &= \Prox_{\mu F^*}( \Ga^k + \mu K(\tilde \Si^k), \\
	\Si^{k+1} &= \Prox_{\tau H}(  \Si^k-\tau K^*(\Ga^{k+1}) ), \\
	\tilde \Si^{k+1} &= \Si^{k+1} + \theta (\Si^{k+1} - \Si^k) ,
\end{align*}
where $\theta\in[0;1]$ and the two other parameters should satisfy $\mu\tau \norm{K}^2< 1$ where $\norm{K}$ is the spectral norm of the operator $K$. Under these conditions, it is shown in~\cite{Chambolle11}  that $\Sigma^{k}$ converges to a solution $\Sigma^\star$ of~\eqref{eq-relaxed-regularized-cvx}.

%\todo{ I did not understand this : The norm of operator $K$ can be bounded as $\norm{K}^2\leq 1+ \norm{G^* G}_{\infty}.\norm{Y}^2$ (what is $\norm{\cdot}_\infty$?) Furthermore, unless this bound is tight,  I would rather use a few power iterations to approximate $\norm{K}$.  }

% Due to the form of $K$, it may be interesting to look at preconditionning techniques...

